The Devils in The Details: Placing Decoy Routers in the Internet

Decoy Routing, the use of routers (rather than end hosts) as proxies, is a new direction in anti-censorship research. Decoy Routers (DRs), placed in Autonomous Systems, proxy traffic from users; so the adversary, e.g., a censorious government, attempts to avoid them. It is quite difficult to place DRs so the adversary cannot route around them for example, we need the cooperation of 850 ASes to contain China alone. In this paper, we consider a different approach. We begin by noting that DRs need not intercept all the network paths from a country, just those leading to Overt Destinations, i.e., unfiltered websites hosted outside the country (usually popular ones, so that client traffic to the OD does not make the censor suspicious. Our first question is; How many ASes are required for installing DRs to intercept a large fraction of paths from, e.g., China to the top n websites (as per Alexa)? How does this number grow with n? Few ASes (approx. 30) intercept over 90% of paths to the top n sites, for n = 10, 20...200. Our first contribution is to demonstrate with real paths that the number of ASes required for a world-wide DR framework is small (approx. 30). Further, censor nations attempts to filter traffic along the paths transiting these 30 ASes will not only block their own citizens, but others residing in foreign ASes. Our second contribution in this paper is to consider the details of DR placement: not just in which ASes DRs should be placed to intercept traffic, but exactly where in each AS. We find that even with our small number of ASes, we still need a total of about 11,700 DRs.We conclude that, even though a DR system involves far fewer ASes than previously thought, it is still a major undertaking. For example, the current routers cost over 10.3 billion USD, so if DR at line speed requires all new hardware, the cost alone would make such a project unfeasible for most actors.

==> sections/scratch.tex <==
\subsection{Qi Points: The Algorithm}

In brief, our placement strategy is to select "key" ASes that appear in a large number of paths leading to important sites on the web \emph{i.e.} potential overt destinations. We then find key routers inside the key ASes. 

We present it as a formal algorithm in Algorithm 1.

\begin{algorithm}
\label{alg:odsp}
\begin{algorithmic}
\Procedure{FindAS}{ List of Websites $WList$, Routing Tables $RT$, Threshold $Thold = 0.9$} 
\Comment Routing Tables are from RouteViews. Target Websites are from Alexa.
\State PathList  = (empty list), ASList = (empty list)
\For{every website $w_i$ in $WList$}
\State \textbf{Find} $w_i.p$, the prefix corresponding to $w_i$
\State PathList.append ( ExtendPath($RT$, $w_i.p$) )
\State Add all new AS found to ASList
\EndFor
\Comment ExtendPath uses Gao's algorithm. We compute the paths to prefix $w_i.p$ using the routing information in $RT$.
\State \textbf{Sort} ASList by frequency with which ASes appear in paths of PathList
\State \textbf{Return} list of most common $k$ ASes, excluding ASes in censorious countries, where $k$ is the smallest number s.t. $k$ ASes cover a fraction of at least $Thold$ of paths (in PathList)
\Comment We find that the list of ASes, that cover $90\%$ of all paths, is quite small - about $30$ ASes.
\EndProcedure
\end{algorithmic}

\begin{algorithmic}
\Procedure{FindRouter}{AS $A$, Threshold $t$} 
\State \textbf{Map} internal structure of AS $A$ with Rocketfuel
\State \textbf{Remove} aliases with MIDAR
\State \textbf{Sort} routers by frequency with which they appear in traceroute traces.
\State \textbf{return} list of most common $k$ routers, where $k$ is the smallest number s.t. $k$ routers cover a fraction of at least $t$ of traces through the AS.
\EndProcedure
\end{algorithmic}
\caption{Qi Points: AS and Router selection}
\end{algorithm}

%\begin{enumerate}
%\item For all websites W in the list (say, Alexa top 100):

%\begin{enumerate}
%\item Find P, the IP prefix of W.

%\item Find all possible paths from prefix P to every other AS, using the algorithm of Gao and Qiu. 
%(BGP RIBs can be obtained from RouteViews, and Inter-AS relationships, from %CAIDA~\cite{caida-inter-as-rels}.)
%\end{enumerate}

%\item Using the paths obtained in the previous step, sort the ASes in descending %order of path frequency (i.e. the number of times they appear in the paths).

%\item Select the top ASes of this list as key ASes in the Internet.

%\item For each chosen AS, generate a map of the internal structure of the AS, using Rocketfuel.

%\item Select the routers which appear in a large number of \texttt{traceroute} %paths as key routers of the key AS. These  are the ones which should be replaced by DRs.
%\end{enumerate} 






RESULTS.

In some large multinational network providers (such as AS174, corresponding to Cogent Communications), that have over $1700$, only around $300$ routers appear in almost all the discovered network paths. In others, such as large scale web and cloud service providers (\emph{e.g.} AS16509, corresponding to Amazon.com), a total of $4644$ routers ($1056$ edge + $3588$ core routers) are needed to achieve a cover of $90\%$ of the discovered paths. 



GAO's  ALGORITHM.


\begin{algorithm}[h!]
\caption{Gao's Prefix-to-AS Path Estimation Algorithm \cite{gao2001inferring}}
\begin{small}
\begin{algorithmic}
\Procedure{Gao\_algorithm}{BGP paths $RIB\_file$, AS relationships $CAIDARels$, list of prefixes $PrefixInput$} 
%\Comment Topology Construction Phase
\State \textbf{declare} $PathSet$ \Comment Paths to a chosen prefix from an AS.
\State \textbf{declare} $Frequency\_Index$ \Comment Counts times a sure path appears in $RIB\_file$
\State \textbf{declare} $Uncertainty\_count$ \Comment Counts ASes appended to a sure path. 

\For{every prefix $p \in PrefixInput$}
 \State \textbf{Select} all sure paths (for $p$) from $RIB\_file$.
 \State \textbf{Inspect} each sure path for possible extension (satisfying Valley-Free and Loop-Free properties). \Comment To find business relationship with $k^{th}$ AS of path, we use $CAIDARels$.
 \For{every sure path $sp$ that is extended}
 	\State $PathSet$ = $PathSet \cup sp$
    \State \textbf{Increment} path length of $sp$, $Uncertainty\_count$  
  \EndFor
 \EndFor

\For{every prefix $p \in PrefixInput$}
  \For{every AS $A(i)$ with a path to $p$}
   \State \textbf{sort} all paths from $A(i)$ to $p$, as follows:
      \If{Unique shortest path}
      \State \textbf{select} path for final topology.
      \Else \If{Multiple shortest paths}
      \State \textbf{select} path with least $Uncertainty\_count$ for final topology.
      \Else 
        \State \textbf{select} path with maximum $Frequency\_Index$ for final topology.
        \EndIf
        \EndIf
      \EndFor
\EndFor

\EndProcedure

\end{algorithmic}
\end{small}
\label{alg:gao}
\end{algorithm}


